CodeSift: An LLM-Based Reference-Less Framework for Automatic Code Validation

The advent of large language models (LLMs) has greatly facilitated code generation, but ensuring the functional correctness of generated code remains a challenge. Traditional validation methods are often time-consuming, error-prone, and impractical for large volumes of code. We introduce CodeSift, a novel framework that leverages LLMs as the first-line filter of code validation without the need for execution, reference code, or human feedback, thereby reducing the validation effort. We assess the effectiveness of our method across three diverse datasets encompassing two programming languages. Our results indicate that CodeSift outperforms state-of-the-art code evaluation methods. Internal testing conducted with subject matter experts reveals that the output generated by CodeSift is in line with human preference, reinforcing its effectiveness as a dependable automated code validation tool.

==> body/examples/first.tex <==
result = []
for number in numbers:
    if number not in result:
        result.append(number)
return result

==> body/examples/snoopy.tex <==
#!/bin/bash
usermod -L snoopy

==> body/execution_evaluation.tex <==
\subsection{Execution-Based Accuracy}
We set up a sandbox testing environment with Podman containers hosting Redhat UBI images to execute the generated bash scripts.
Our execution contains six steps, including 
1) Pre-checking, i.e., checking the syntax correctness of the generated code, 
2) prologue setup, e.g., launch a container and create a user with a home directory,
3) generated code execution, 
4) epilogue examination, e.g., filesystem changes,
5) evaluation to determine the code execution correctness, 
6) cleanup to remove the container.
We check if the generated code is correct by examining its syntax, execution accuracy, and the potential collateral impact on the filesystem. 
Any errors reported by the \texttt{bash -n} command or in the \texttt{stderr} output, as well as any unexpected changes or absence of expected changes in the filesystem, will be deemed as failures. Table~\ref{tab:example_execution} shows a detailed example of the six steps of the execution-based evaluation.


\begin{table}[ht]
\scriptsize
\centering
\caption{Examples illustrating the six steps of Execution-based accuracy.}
\label{tab:example_execution}
\begin{tblr}{
        hline{1,Z}={1pt},
        hline{2-9}={solid},
        colspec={X[-1,l]|X[3,l]},
        rows={m,rowsep=0pt},
        row{1}={m,bg=cyan!5,fg=black},
        row{2}={m,bg=cyan!8,fg=black},
        row{3}={m,bg=yellow!10,fg=black},
        row{4}={m,bg=yellow!15,fg=black},
        row{5}={m,bg=yellow!20,fg=black},
        row{6}={m,bg=yellow!25,fg=black},
        row{7}={m,bg=yellow!30,fg=black},
        row{8}={m,bg=yellow!35,fg=black},
    }
\textbf{Input Task} & What is the bash command to lock user snoopy's account?\\
\textbf{Generated code} & 
\begin{minipage}{0.3\columnwidth}
\inputminted[fontsize=\scriptsize]{bash}{body/examples/snoopy.tex}
\end{minipage}\\
\textbf{Pre-checking}       & Syntax checking the generated code with the \texttt{bash -n} command.\\
\textbf{Prologue}           & Launch a container with the \texttt{podman run} command, create a user called snoopy with the \texttt{useradd snoopy} command, and set password for snoopy with the \texttt{sed -i} \texttt{\textquotesingle{}/\string^snoopy:/s+:!!:+:\$-\$Woodstock:+\textquotesingle{}} \texttt{/etc/shadow} command.
\\
\textbf{Execution}          & Executing the generated code.\\
\textbf{Epilogue}           & Check any filesystem changes excluding those expected ones. For example, ignore any changes in \texttt{/etc\$/d}, \texttt{/etc/.pwd.lock\$/d}, \texttt{/etc/passwd\$/d}, etc. \\
\textbf{Evaluation}         & {\begin{itemize}[leftmargin=*]
\item Check any errors in the \texttt{stderr}.\\
\item Check whether the snoopy account still exists by checking the absence of the \texttt{snoopy:x:1001:1001::/home/snoopy:/bin/bash} line in the \texttt{/etc/passwd} file.\\ 
\item Check whether the snoopy account is locked by checking the absence of the \texttt{snoopy:!$-$Woodstock:19790:0:99999:7:::} or \texttt{snoopy:!!$-$Woodstock:19790:0:99999:7:::} line in the \texttt{/etc/shadow}
file.\\
\item Check any collateral filesystem change.
\end{itemize}}\\
\textbf{Cleanup}            & Shutdown the container with the \texttt{podman rm} command.\\
\end{tblr}
\end{table}

% syntax checking
% executing checking => no runtime error in stderr
% functionality checking => snoopy is locked 
% side effect checking => no additional ops


==> body/extra.tex <==
% \begin{table}[]
% \begin{tabular}{|l|l|ll|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Code Generation Models}} & \multicolumn{1}{c|}{\multirow{2}{*}{Correct}} & \multicolumn{2}{c|}{Incorrect}                         \\ \cline{3-4} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{l|}{syntax\_error} & functional\_error \\ \hline
% starcoder                                       & 514                                           & \multicolumn{1}{l|}{281}           & 845               \\ \hline
% llama2chat                                      & 405                                           & \multicolumn{1}{l|}{855}           & 380               \\ \hline
% codellama                                       & 786                                           & \multicolumn{1}{l|}{312}           & 542               \\ \hline
% mistral                                         & 599                                           & \multicolumn{1}{l|}{598}           & 443               \\ \hline
% \end{tabular} 
% \label{tab:stats}
% \caption{Dataset Statistics}
% \end{table}

% \begin{table*}[]
% \centering
% \begin{tabular}{|ll|llll|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Methods}}}                                                                                                                                                 & \multicolumn{4}{c|}{\textbf{Code Generation models}}                                                                 \\ \cline{3-6} 
% \multicolumn{2}{|c|}{}                                                                                                                                                                         & \multicolumn{1}{l|}{starcoder} & \multicolumn{1}{l|}{llama2chat} & \multicolumn{1}{l|}{codellama} & mistral \\ \hline
% \multicolumn{1}{|l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Baseline \\ (mistral as evaluator)\end{tabular}}} & Single Grading                                                       & \multicolumn{1}{l|}{64.32}     & \multicolumn{1}{l|}{70.00}      & \multicolumn{1}{l|}{56.15}     & 61.00   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & Reference Grading                                                    & \multicolumn{1}{l|}{68.65}     & \multicolumn{1}{l|}{70.00}      & \multicolumn{1}{l|}{58.06}     & 60.00   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & \begin{tabular}[c]{@{}l@{}}Embedding-based\\ Similarity\end{tabular} & \multicolumn{1}{l|}{65.12}     & \multicolumn{1}{l|}{38.48}      & \multicolumn{1}{l|}{68.23}     & 46.22   \\ \hline
% \multicolumn{1}{|l|}{\multirow{3}{*}{Similarity Analysis}}                                                              & mistral (as evaluator)                                                              & \multicolumn{1}{l|}{71.40}     & \multicolumn{1}{l|}{53.10}      & \multicolumn{1}{l|}{73.29}     & 56.34   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & mixtral                                                              & \multicolumn{1}{l|}{62.92}     & \multicolumn{1}{l|}{51.64}      & \multicolumn{1}{l|}{64.20}     & 54.63   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & llama2chat                                                           & \multicolumn{1}{l|}{52.15}     & \multicolumn{1}{l|}{36.82}      & \multicolumn{1}{l|}{54.57}     & 41.03   \\ \hline
% \multicolumn{1}{|l|}{\multirow{3}{*}{Difference Analysis}}                                                              & mistral                                                              & \multicolumn{1}{l|}{61.03}     & \multicolumn{1}{l|}{55.54}      & \multicolumn{1}{l|}{53.29}     & 60.06   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & mixtral                                                              & \multicolumn{1}{l|}{60.36}     & \multicolumn{1}{l|}{51.03}      & \multicolumn{1}{l|}{61.89}     & 56.15   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & llama2chat                                                           & \multicolumn{1}{l|}{57.68}     & \multicolumn{1}{l|}{53.59}      & \multicolumn{1}{l|}{52.68}     & 54.14   \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}CodeSift\\ Essemble Synthesis\end{tabular}}}            & mistral                                                              & \multicolumn{1}{l|}{72.92}     & \multicolumn{1}{l|}{66.21}      & \multicolumn{1}{l|}{65.18}     & 66.76   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & mixtral                                                              & \multicolumn{1}{l|}{67.56}     & \multicolumn{1}{l|}{57.86}      & \multicolumn{1}{l|}{65.42}     & 60.30   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & llama2chat                                                           & \multicolumn{1}{l|}{62.85}     & \multicolumn{1}{l|}{57.56}      & \multicolumn{1}{l|}{54.63}     & 55.60   \\ \cline{2-6} 
% \multicolumn{1}{|l|}{}                                                                                                  & cross-LLMs                                                           & \multicolumn{1}{l|}{75.36}     & \multicolumn{1}{l|}{62.32}      & \multicolumn{1}{l|}{70.79}     & 63.90   \\ \hline
% \end{tabular}
% \caption{Accuracy of various LLM-based Code Evaluation methods} \label{tab:main_results}
% \end{table*}



% \textit{RQ1: What is the impact of different phases of CodeSift on its validation accuracy?} The impact of different phases of CodeSift on its validation accuracy was assessed through an analysis of the results obtained from the semantic inference phase and the difference analysis phase, as presented in Table~\ref{tab:phases}. Across the four datasets, our findings indicate that the LLM-evaluators exhibited a higher capability in identifying semantic similarity compared to difference analysis. Upon manual inspection of the data, it was observed that the generated code-text often lacked comprehensive details regarding the range and scope of the code, posing challenges for the models to accurately identify differences. Notably, the Mixtral model demonstrated superior performance in identifying discrepancies between the task and code-text compared to other LLM-evaluators.
% Notably, we delve into a comprehensive examination of the code-to-text phase, recognizing its pivotal role in the overall process.

% \begin{table*}[]
% \begin{tabular}{|l|cc|ll|ll|}
% \hline
% Evaluator LLMs                 & \multicolumn{2}{c|}{mistral}                                                                                                                        & \multicolumn{2}{c|}{mixtral}                                                                                                                                             & \multicolumn{2}{c|}{llama2}                                                                                                                                     \\ \hline
% \multicolumn{1}{|c|}{Code Generation Models} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Similarity\\ Inference\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Difference\\ Analysis\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Similarity\\ Inference\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ Analysis\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Similarity\\ Inference\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ Analysis\end{tabular}} \\ \hline
% starcoder                      & \multicolumn{1}{c|}{\textbf{71.40}}                                                 & 61.03                                                         & \multicolumn{1}{l|}{62.92}                                                          & \textbf{60.36}                                                                     & \multicolumn{1}{l|}{52.15}                                                          & 57.68                                                                              \\ \hline
% llama2chat                     & \multicolumn{1}{c|}{\textbf{53.10}}                                                 & \textbf{55.54}                                                & \multicolumn{1}{l|}{51.64}                                                          & 51.03                                                                              & \multicolumn{1}{l|}{36.82}                                                          & 53.59                                                                              \\ \hline
% codellama                      & \multicolumn{1}{c|}{\textbf{73.29}}                                                 & 53.29                                                         & \multicolumn{1}{l|}{64.20}                                                          & \textbf{61.89}                                                                     & \multicolumn{1}{l|}{54.57}                                                          & 52.68                                                                              \\ \hline
% mistral                        & \multicolumn{1}{c|}{\textbf{56.34}}                                                 & \textbf{60.06}                                                & \multicolumn{1}{l|}{54.63}                                                          & 56.15                                                                              & \multicolumn{1}{l|}{41.03}                                                          & 54.14                                                                              \\ \hline
% \end{tabular} \label{tab:phases}
% \caption{Phase level accuracy across various LLMs as evaluators}
% \end{table*}

%\textit{RQ2: What is the agreement percentage between the evaluations conducted by CodeSift and those obtained through test case-based validation techniques?} We focus on the hybrid model and compare it with ground truth.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
Methods                         & evaluator\_llm & codellama & mistral \\ \hline
\multirow{2}{*}{judge\_llm}     & mistral        &           &         \\ \cline{2-4} 
                                & llamachat      &           &         \\ \hline
\multirow{2}{*}{ICE}            & mistral        & 60        &         \\ \cline{2-4} 
                                & llamachat      &           &         \\ \hline
\multirow{2}{*}{codeSift\_Sim}  & mistral        & 65        &         \\ \cline{2-4} 
                                & llamachat      &           &         \\ \hline
\multirow{2}{*}{codeSift\_diff} & mistral        &           &         \\ \cline{2-4} 
                                & llamachat      &           &         \\ \hline
\multirow{2}{*}{essemble}       & mistral        &           &         \\ \cline{2-4} 
                                & llamachat      &           &         \\ \hline
\end{tabular}
\end{table}

==> body/intro.tex <==
\section{Introduction}

In today's software development landscape, the proliferation of large language models (LLMs) has vastly accelerated the pace of code generation across various domains. %from web development to machine learning applications. 
The widespread adoption of generated code brings a need for robust validation mechanisms to ensure its functional correctness before deployment in production systems. Deploying unvalidated code directly into these systems can lead to severe consequences, including performance degradation and critical system failures. While manual inspection offers insights, the sheer volume of generated code makes it labor-intensive and time-consuming.

Recent approaches to evaluate generated code either use reference codes to compare with or are based on runtime execution correctness~\cite{eghbali2023crystalbleu,ren2020codebleu, zhou2023codebertscore, dong2023codescore,du2023classeval,schafer2024testgen}. However, these approaches come with the need for availability of reference codes and are limited by scalability constraints with increased workload which hinders their applications in real world systems.

%Many approaches to evaluate generated code have been proposed along three dimensions: (1) match-based~\cite{papineni2022bleu,eghbali2023crystalbleu,ren2020codebleu} (2) embedding-based  ~\cite{zhang2020bertscore,zhou2023codebertscore} and (3) execution-based~\cite{kulal2019spoc,chen2021codex,hendrycks2021measuring,dong2023codescore,du2023classeval,schafer2024testgen,chen2022codet}. Despite their capacity to process extensive datasets, match-based and embedding-based approach's accuracy is compromised by the absence of code semantic validation and function correctness checking. Also, there is a requirement for the reference code to be available, hindering their practicability. While effective, execution-based approaches are inherently limited by scalability constraints with increased workload. 
% On the other hand, existing LLM-based evaluation approaches target solely text data~\cite{zheng2023judging}. 

To address these issues, we propose a novel framework, called CodeSift, to act as a first-line filter for generated code evaluation. This framework is designed to validate the functional correctness of generated code using LLMs as evaluators. By harnessing the power of advanced natural language understanding, semantic comprehension, and code analysis capabilities offered by LLMs, %~\cite{li2023starcoder,jiang2023mistral,touvron2023llama,roziere2023code} 
 %and rule-based code syntax checking abilities~\cite{pylint}, 
 CodeSift offers a scalable and efficient solution to the challenge of code validation, significantly reducing the burden on human validators and streamlining the code validation process. Code snippets that pass the first-line validation can undergo further scrutiny by human experts or be tested in a controlled development environment, thus maximizing efficiency and minimizing the risk of deploying faulty code%, thereby accelerating the widespread adoption of generated code in real-world applications. 
 Our contributions are: (1) We propose CodeSift, a novel and effective framework for first-line evaluation of generated code, eliminating the need for execution, reference codes, and test cases. (2) We demonstrate CodeSift's effectiveness in achieving concordance with conventional test case-based validation techniques and emphasizing the importance of separately capturing similarities and differences for accurate labeling of generated code.%We demonstrate the effectiveness of LLMs in detecting various functional issues within code, such as logical errors, syntax errors, and absent functions.demonstrate the utility of CodeSift by comparing different code LLMs, particularly when reference code or test cases are unavailable. % such as AIOPS, Code translation, etc []. 

==> body/intro_backup.tex <==
\section{Introduction}

In today's software development landscape, the proliferation of large language models (LLMs) has vastly accelerated the pace of code generation across various domains, from web development to machine learning applications. However, the widespread adoption of generated code inevitably and inherently brings a pressing need for robust validation mechanisms to ensure its functional correctness before deployment in production systems. Deploying unvalidated code directly into production systems can lead to severe consequences, including performance degradation and critical system failures. While manual inspection offers insights, the sheer volume of generated code makes it labor-intensive and often impractical for human experts to validate manually.

Match-based code evaluation approaches~\cite{papineni2022bleu,eghbali2023crystalbleu,ren2020codebleu} and embedding-based code evaluation approaches~\cite{zhang2020bertscore,zhou2023codebertscore} measure the resemblance between generated and reference code through techniques like n-gram matching or token embedding cosine similarities. Despite their capacity to process extensive datasets, their accuracy is compromised by the absence of code semantic validation and function correctness checking. Moreover, the match-based approaches only work when reference code is available, hindering their practicability.

Execution-based code evaluation approaches~\cite{kulal2019spoc,chen2021codex,hendrycks2021measuring,dong2023codescore} involve running the generated code against a predefined set of test cases and comparing the output with expected results. 
While effective, they are inherently limited by scalability constraints. These limitations are mitigated by automated test case generation techniques~\cite{du2023classeval,schafer2024testgen,chen2022codet,codamosa2023,tufano2022test,mastropaolo2022using}. 
However, validating the generated test cases increases the workload, rendering the entire execution-based approach impractical.



In this context, our proposed framework, CodeSift, serves as a crucial first-line filter. CodeSift is a novel framework for validating the functional correctness of generated code using LLMs as evaluators. By harnessing the power of advanced natural language understanding, semantic comprehension, and code analysis capabilities offered by LLMs, our framework offers a scalable and efficient solution to the challenge of code validation, significantly reducing the burden on human validators and streamlining the code validation process. Code snippets that pass the initial validation can then undergo further scrutiny by human experts or be tested in a controlled development environment, thus maximizing efficiency and minimizing the risk of deploying faulty code, thereby accelerating the widespread adoption of generated code in real-world applications. Our contributions are as follows: (1) % such as AIOPS, Code translation, etc []. 

==> body/metric_table.tex <==
\begin{table*}[]
\caption{Comparison of CodeSift with State-of-the-Art Code Evaluation Metrics. CodeSift's effectiveness in ranking various code generation models is demonstrated. We consider the metric number closest to the execution accuracy as the best.}
\label{tab:metric_results}
\centering
\scriptsize
\begin{tblr}[]{
        hline{1,4,Z}={1pt},
        hline{2} = {solid},
        vline{1,2,Z}={1pt},
        vline{6,7}={solid},
        rows={m,rowsep=0pt},
        colspec={X[-1,l]X[-1,l]X[-1,l]X[-1,c]X[-1,c]X[-1,c]X[-1,c]X[-1,c]X[-1,c]X[-1,c]},
        cell{1}{1} ={r=3}{c},
        cell{1}{2}={c=9}{c},
        cell{2}{2,7}={c=4}{c},
        cell{even[4-Z]}{1-Z}  = {bg=gray!10},
        cell{4-Z}{1} = {font=\bfseries},
        row{2} = {font=\bfseries},
        cell{4}{2-Z} = {fg=blue},
        cell{9}{2,5,9} = {font=\bfseries},
        cell{7}{3,8} = {font=\bfseries},
        cell{6}{4,7,10} = {font=\bfseries},
        cell{8}{6} = {font=\bfseries}
}
\textbf{Metrics }   &  \textbf{Dataset with Code Generation Models} &&&& &&&\\
                    & HumanEval (Python) &&&                           & Bash      & MBPP (Python) &&& \\
                    &  Starcoder & GPT3.5   &  Codellama   &  Mistral  & Codellama &  Starcoder & GPT3.5   &  Codellama   &  Mistral    \\  
Execution Accuracy  &  31.3      & 71.3     &  52.1        &  36.5     & 54.4      &  54.88     & 79.6     &  65.4        &  50.3       \\  
CodeBLEU~\cite{ren2020codebleu}            &  15.3      & 29.2     &  24.02       &  26.1     & NA        &  17.84     & 22.7     &  22.5        &  20.7       \\  
ICE-Score~\cite{zhuo2024icescore}           &  45.3      & 51.5     &  52.7        &  51.4     & 83.3      &  49.8      & 51.3     &  50.3        &  50.6       \\  
CodeBertScore~\cite{zhou2023codebertscore}       &  76.1      & 79.3     &  80.1        &  80.4     & NA        &  78.6      & 81.1     &  81.6        &  81.3       \\  
Rouge\_L~\cite{lin2004rouge}             &  37.02     & 36.8     &  43.9        &  38.9     & 62.1      &  44.2      & 38.6     &  42.6        &  43.1       \\  
CodeSift Ensemble   &  28.3      & 60.7     &  47.9        &  35.9     & 44.4      &  61.9      & 71.1     &  72.6        &  66.1       \\
\end{tblr}
\end{table*}

==> body/relatedwork_short.tex <==
\section{Related work}
%In recent years, the field of code generation has witnessed significant advancements, driven largely by the emergence of LLMs and deep learning techniques. 
Many approaches for generated code evaluation have been proposed in the literature along three dimensions: (1) Match-based: BLEU and CrystalBLEU are commonly used metrics~\cite{papineni2022bleu, eghbali2023crystalbleu}, calculated based on n-gram matching.  (2) Embedding-based: CodeBertScore, for example, ~\cite{zhou2023codebertscore} measures the similarity between generated and reference code using token embeddings and by incorporating contextual information. and (3) Execution-based: Execution-based evaluation approaches evaluate code quality based on runtime execution correctness using the pass@$k$ metric where $k$ is the number of generated code samples~\cite{kulal2019spoc,chen2021codex}. APPS~\cite{hendrycks2021measuring} and CodeScore~\cite{dong2023codescore} evaluate functional correctness using the PassRatio metric, calculating the average fraction of test cases passed. Other code evaluation approaches calculate the statistical possibility of AST nodes~\cite{palacio2023evaluating} and evaluate class-level code generation~\cite{du2023classeval}. 

While these approaches are effective, these methods lack semantic validation and functional correctness, which could potentially improve performance. The match and embedding-based approaches only work when reference code is available, hindering their practicability. 
Validating the generated test cases increases the workload, rendering the execution-based approach impractical.
To address these issues, and inspired by LLM-based evaluation methods for text data~\cite{zheng2023judging}, we introduce CodeSift that uses LLMs as a first-line filter to validate the functional correctness of the generated code. %On the other hand, existing LLM-based evaluation approaches target solely text data~\cite{zheng2023judging}. %Regardless of their limited capabilities in code, they have brought to light the opportunities of evaluating code on text dimension. 







==> body/todo.tex <==
write about syntax checking and fixing the syntax through llm
add example


architecture diagram

llms used are open source

expand RQ3


Intro - expand on contributions

experiments:
we do strict marking -- not partially correct
